Reality's Canvas, Language's Brush: Crafting 3D Avatars from Monocular Video

Recent advancements in 3D avatar generation excel with multi-view supervision for photorealistic models. However, monocular counterparts lag in quality despite broader applicability. We propose ReCaLaB to close this gap. ReCaLaB is a fully-differentiable pipeline that learns high-fidelity 3D human avatars from just a single RGB video. A pose-conditioned deformable NeRF is optimized to volumetrically represent a human subject in canonical T-pose. The canonical representation is then leveraged to efficiently associate neural textures using 2D-3D correspondences. This enables the separation of diffused color generation and lighting correction branches that jointly compose an RGB prediction. The design allows to control intermediate results for human pose, body shape, texture, and lighting with text prompts. An image-conditioned diffusion model thereby helps to animate appearance and pose of the 3D avatar to create video sequences with previously unseen human motion. Extensive experiments show that ReCaLaB outperforms previous monocular approaches in terms of image quality for image synthesis tasks. Moreover, natural language offers an intuitive user interface for creative manipulation of 3D human avatars.

==> figs/teaser.tex <==

\makeatletter
\g@addto@macro\@maketitle{
  \begin{figure}[H]
  \setlength{\linewidth}{\textwidth}
  \setlength{\hsize}{\textwidth}
  \centering
    \includegraphics[width=\linewidth]{figs/teaser.pdf}
    \vspace{-5mm}
	\caption{\textbf{Overview of \OURS{}.} We propose \OURS{}, a novel approach for photo-realistic 3D avatar creation from monocular video and different types of manipulations. Our approach models neural humans with a disentangled neural texture field and enables different types of manipulation, including novel view rendering, novel pose animation, and novel appearance with customized shape, texture, and illumination by language brush.}%\Yuchen{\textbf{Overview of \OURS{}.} We propose \OURS{}, a new approach for 3D avatar creation and manipulation from a single monocular input video. It generates an animatable human avatar for novel view and novel pose scenarios, which can be edited on shape, texture and illumination.}} 
    \label{fig:teaser}
    \vspace{-2mm}
	\end{figure}
}
\makeatother

